TRACE: Training-aware Robustness and Challenge Evaluation for Text-Vision Embedding Models

Existing benchmarks for text-vision embedding models report aggregate scores that obscure whether performance comes from general capabilities, task-specific adaptation, or robustness to challenging tasks. We introduce TRACE, a Training-aware Robustness and Challenge Evaluation framework that reorganizes 168 tasks from various sources of datasets into three categories: General, Adaptability, and Challenge. Through controlled experiments on two text-vision embedding models, we show that combining general and adaptation data improves Adaptability performance by 7.67 and 7.09 points, respectively, while largely preserving General performance. However, Challenge performance remains below 5.0, with limited improvements from additional training data. Further analysis identifies multilingual and visual-document tasks as major weaknesses. Our findings demonstrate that data adaptation alone is insufficient to address these challenges, highlighting the need for methodological advances beyond data-centric improvements.

==> accv/1.tex <==
\section{Introduction}
\label{sec:introduction}

CLIP-style vision-language models map images and texts into a shared embedding space, enabling applications such as image-text retrieval, visual question answering, clustering, and multimodal search~\cite{}.
%
Although large CLIP models show strong performance, their computational cost limits their use in real-world settings such as mobile devices, edge deployment, and low-latency retrieval systems.
%
This has motivated recent work on small CLIP models, which aim to preserve the capability of large vision-language models with substantially fewer parameters.

A common approach for building small CLIP models is knowledge distillation.
%
Methods such as CLIP-KD~\cite{} and TinyCLIP~\cite{} transfer knowledge from a large teacher model to a compact student and achieve competitive results on standard retrieval benchmarks.
%
However, existing evaluations are still largely retrieval-centered.
%
While retrieval is important, it does not fully reflect whether small CLIP models are robust across broader vision-language embedding tasks.
%
This leaves an important question open: do current small CLIP models generalize beyond the tasks and datasets commonly used to train and evaluate them?

Recent benchmarks such as MMEB~\cite{} and MIEB~\cite{} provide broader evaluation suites for multimodal embedding models, covering diverse task types beyond conventional retrieval.
%
However, aggregate benchmark scores are difficult to interpret without considering the relationship between training and evaluation data.
%
A model may perform well because the task is generally solvable from large-scale pretraining, because related in-domain training data is available, or because the evaluation set is close to the training distribution.
%
This issue is especially critical for small CLIP models, whose limited capacity may make them more sensitive to data selection.
%
Therefore, evaluating small CLIP models requires not only broader benchmarks, but also a training-aware protocol that explains where the performance comes from.

In this work, we propose \textbf{TRACE}, a \textbf{Training-aware Robustness and Challenge Evaluation} framework for small CLIP models.
%
TRACE organizes training and evaluation data according to their dataset-level relationship and separates evaluation into three groups.
%
The \textbf{General} group measures tasks that can be addressed using common image-text training data such as CC12M~\cite{} and DataComp~\cite{}.
%
The \textbf{Adaptability} group measures tasks where related in-domain training data is available from recent embedding benchmarks such as MMEB and MIEB.
%
The \textbf{Challenge} group contains evaluation tasks that remain below a fixed performance threshold and do not have related training data.
%
This design allows us to distinguish general vision-language alignment, dataset-level adaptation, and unresolved out-of-domain limitations.

We instantiate TRACE with two representative small CLIP distillation frameworks, CLIP-KD~\cite{} and TinyCLIP~\cite{}, both with fewer than 40M parameters.
%
For each model, we follow its original training recipe and change only the training data according to the proposed TRACE protocol.
%
We evaluate on MMEB v1--v3 and MIEB, excluding video and audio tasks, and report the original metrics defined by each benchmark or dataset.
%
Our results show that \textbf{Model X} improves by \textbf{Y} on the Adaptability group after training with related data, but achieves only \textbf{Z} improvement on the Challenge group.
%
This demonstrates that benchmark gains can reflect in-domain adaptation, while some tasks remain genuinely challenging for current small CLIP training recipes.

We summarize the contributions of this paper as follows.
%
\begin{itemize}
\item \textbf{Data:} We propose a training setup that separates general training data from benchmark-related in-domain data, enabling clearer analysis of generalization and adaptation.


\item \textbf{Evaluation:} We introduce TRACE, a training-aware evaluation framework that interprets MMEB and MIEB results according to the relationship between training and evaluation data.

\item \textbf{Study:} We conduct a controlled study of CLIP-KD and TinyCLIP to identify which tasks are solvable by general training, which require in-domain adaptation, and which remain challenging.


\end{itemize}


==> accv/2.tex <==
\section{Related Work}
\label{sec:related-work}

\subsection{Small CLIP and Efficient Vision-Language Models}

CLIP-style models learn transferable vision-language representations by aligning images and texts in a shared embedding space~\cite{}.
%
While large CLIP models show strong performance across retrieval and zero-shot recognition, their computational cost limits their use in resource-constrained settings.
%
This has motivated recent work on efficient CLIP training and compact CLIP architectures.

Several studies aim to reduce the cost of CLIP pretraining.
%
EfficientCLIP~\cite{}, RECLIP~\cite{}, and FastCLIP~\cite{} improve training efficiency through data filtering, progressive resolution training, or optimization strategies.
%
Data-centric efforts such as LAION~\cite{} and DataComp~\cite{} further show that the choice and quality of image-text data strongly affect downstream performance.
%
These works highlight the importance of both efficient training and data design for practical vision-language models.
%
Another direction builds small CLIP models through knowledge distillation.
%
CLIP-KD~\cite{} studies different distillation objectives for transferring knowledge from a large CLIP teacher to a compact student.
%
TinyCLIP~\cite{} improves compact CLIP training with affinity mimicking and weight inheritance.
%
MobileCLIP~\cite{} and ComKD-CLIP~\cite{} further explore efficient architectures and comprehensive distillation strategies for small vision-language models.
%
These methods demonstrate that compact CLIP models can achieve strong efficiency-performance trade-offs.

However, most small CLIP studies are still evaluated mainly on retrieval and zero-shot classification benchmarks, such as MS-COCO, Flickr30K, and ImageNet.
%
Although these benchmarks are useful, they do not fully reveal whether small CLIP models are robust across broader vision-language embedding tasks.
%
Moreover, prior work rarely analyzes how the relationship between training and evaluation data affects the reported performance.
%
Our work addresses this gap by evaluating small CLIP models with a controlled, training-aware protocol.

\subsection{Vision-Language Embedding Benchmarks}

Early evaluations of CLIP-style models mainly focused on image-text retrieval and zero-shot classification~\cite{}.
%
These tasks measure basic cross-modal alignment and visual recognition, but they cover only part of the behavior expected from modern embedding models.
%
In real applications, a vision-language embedding model may need to support retrieval, classification, visual question answering, grounding, document understanding, and other matching tasks.

Recent benchmarks have expanded the scope of evaluation.
%
MMEB~\cite{} evaluates multimodal embedding models across diverse task families, including classification, visual question answering, retrieval, and grounding.
%
MMEB-V2~\cite{} and MMEB-V3~\cite{} further extend the benchmark with additional modalities and task settings.
%
MIEB~\cite{} also provides a broad evaluation suite for image and image-text embedding models across many tasks and languages.
%
Together, these benchmarks move beyond retrieval-only evaluation and provide a more comprehensive view of embedding quality.
%
Despite this progress, broad benchmark coverage alone does not fully explain model behavior.
%
A high aggregate score may result from general pretraining, exposure to related in-domain data, or dataset-specific adaptation.
%
This distinction is especially important for small CLIP models, whose limited capacity may make them more sensitive to training data.
%
Existing benchmarks provide diverse evaluation tasks, but they do not explicitly separate generalization, in-domain adaptation, and unresolved challenge cases.

Our work is complementary to these benchmarks.
%
Rather than proposing another task collection, we organize existing benchmark datasets into \textbf{General}, \textbf{Adaptability}, and \textbf{Challenge} groups according to their dataset-level relationship with the training data.
%
This training-aware evaluation protocol allows us to better understand where small CLIP models generalize, where they adapt, and where they still fail.


==> accv/3.tex <==
\section{Method}
\label{sec:method}

We propose \textbf{TRACE}, a \textbf{Training-aware Robustness and Challenge Evaluation} framework for small CLIP models.
%
TRACE evaluates small CLIP models by considering not only their final benchmark scores, but also the relationship between training and evaluation data.
%
The framework has two components: a controlled training setup and a training-aware evaluation protocol.
%
Given existing vision-language embedding benchmarks, TRACE groups tasks into \textbf{General}, \textbf{Adaptability}, and \textbf{Challenge}, then retrains representative small CLIP models under controlled data settings.

\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{figures/trace_pipeline.pdf}
\caption{
Overview of TRACE.
We collect image-text embedding tasks from MMEB and MIEB, remove duplicated datasets and unsupported modalities, group tasks according to their relationship with the training data, and retrain small CLIP models for training-aware evaluation.
}
\label{fig:trace_pipeline}
\end{figure}

\subsection{Benchmark Collection}

We construct our evaluation suite from MMEB v1--v3~\cite{} and MIEB~\cite{}.
%
Since our focus is on image-text embedding models, we exclude video and audio tasks from MMEB-V3.
%
When the same dataset appears in both MMEB and MIEB, we remove the duplicate and keep the MIEB version.
%
The final benchmark contains \textbf{XX} tasks from \textbf{XX} datasets across \textbf{XX} languages.
%
We organize the benchmark at the task level, since the same dataset may support different task formats.
%
For each task, we keep the original evaluation format and metric.

\subsection{Training-Aware Dataset Grouping}

TRACE groups tasks using both dataset-level metadata and controlled model performance.
%
We first check whether each task has related training data in MMEB or MIEB.
%
We then train small CLIP models on broad image-text data and use their performance to identify tasks that can be solved without in-domain data.
%
In this work, we use CLIP-KD~\cite{} and TinyCLIP~\cite{} as performance indicators.
%
All scores are reported on a 0--100 scale.

Let $\tau$ be a fixed performance threshold.
%
For each task $t$, we evaluate the score of a model trained only on general image-text data.
%
A task is considered to have high general performance if its score is greater than or equal to $\tau$.
%
Based on this rule and the availability of related training data, TRACE defines three groups:

\begin{itemize}
\item \textbf{General:}
Tasks whose score after general-data training is greater than or equal to $\tau$.
%
These tasks measure the capability learned from broad image-text data such as CC12M~\cite{} and DataComp-Medium~\cite{}.


\item \textbf{Adaptability:}
Tasks whose score after general-data training is below $\tau$, but related training data is available.
%
These tasks measure whether small CLIP models can benefit from in-domain adaptation.

\item \textbf{Challenge:}
Tasks whose score after general-data training is below $\tau$ and no related training data is available.
%
These tasks measure out-of-domain limitations that cannot be directly addressed by the available benchmark training splits.


\end{itemize}

All validation and test splits are excluded from training.
%
After grouping, TRACE contains \textbf{XX} General tasks, \textbf{XX} Adaptability tasks, and \textbf{XX} Challenge tasks.
%
The General training set contains \textbf{XX} samples from \textbf{XX} datasets, while the Adaptability training set contains \textbf{XX} samples from \textbf{XX} datasets.

\begin{table*}[h!]
\centering
\caption{
Summary of task groups in TRACE.
General tasks are solved by broad image-text training, Adaptability tasks have related training data, and Challenge tasks remain below the threshold without available in-domain training data.
}
\label{tab:trace_groups}
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l c c c l}
\toprule
\textbf{Group} & \textbf{\#Tasks} & \textbf{\#Datasets} & \textbf{\#Train Samples} & \textbf{Purpose} \\ \midrule
General & XX & XX & XX & Basic capability from broad image-text data \\
Adaptability & XX & XX & XX & Adaptation with related training data \\
Challenge & XX & XX & \textemdash & Out-of-domain robustness \\
\bottomrule
\end{tabular}}
\vspace{-2mm}
\end{table*}




\subsection{Model Retraining Protocol}

We instantiate TRACE with CLIP-KD~\cite{} and TinyCLIP~\cite{}, two representative small CLIP distillation frameworks with fewer than 40M parameters.
%
For each method, we keep the original architecture and training objective.
%
The teacher model is fixed across all students, and the only controlled change is the training data.

For the General setting, models are trained on CC12M and DataComp-Medium.
%
For the Adaptability setting, we further include all available training splits from MMEB and MIEB.
%
Each example is represented as an image-text pair, where the text may be a caption, class label, question-answer pair, instruction, or answer choice.
%
We treat all examples as anchor-positive pairs for contrastive learning.
%
Unless otherwise stated, we follow the original hyperparameters of each method.
%
Detailed training settings are provided in Sec.~\ref{sec:experiments}.

\subsection{Task Prefix Instruction}

Different tasks use different text formats.
%
To reduce this mismatch, we use task-specific prefix instructions following MIEB~\cite{}.
%
The prefix is applied during both training and evaluation for all models.

For retrieval, the text describes the target image.
%
For classification, we use the standard CLIP prompt format, such as ``a photo of a {class}''.
%
For visual question answering and multiple-choice tasks, we concatenate the question with each candidate answer.
%
The final prediction is obtained by selecting the text candidate with the highest image-text similarity.
%
We provide an ablation on task prefix instructions in Sec.~\ref{sec:experiments}.

\subsection{Evaluation Protocol}

We evaluate all models using the official MMEB and MIEB evaluation code.
%
For each task, we follow the original benchmark setting and report the official metric.
%
All metrics are reported on a 0--100 scale.
%
We evaluate results separately for the General, Adaptability, and Challenge groups.
%
This allows us to measure whether a small CLIP model learns from broad image-text data, adapts to related training data, or still fails on out-of-domain tasks.


==> accv/4.tex <==
\section{Results}
\label{sec:results}

We organize the results around four questions.
%
First, we compare model performance across the three TRACE groups.
%
Second, we study how well small CLIP models adapt when related training data is available.
%
Third, we analyze why the Challenge group remains difficult.
%
Finally, we measure the gap between small models and the large teacher.

\subsection{Overall Performance across TRACE Groups}

Table~\ref{tab:main_results} reports the main results under TRACE.
%
We compare the original models, models trained only on General data, and models trained with both General and Adaptability data.
%
The results show that \textbf{XXXXXX}.
%
In particular, small CLIP models achieve stronger performance on the General group, suggesting that these tasks can be addressed by broad image-text training.
%
However, the performance is lower on the Adaptability and Challenge groups, showing that retrieval-centered evaluation does not fully capture the robustness of small CLIP models.

\begin{table*}[h!]
\centering
\caption{
Main results under TRACE.
All metrics are reported on a 0--100 scale using the official metric of each benchmark.
}
\label{tab:main_results}
\setlength{\tabcolsep}{3.5pt}
\small
\begin{tabular}{l l | c | c c c }
\toprule
\textbf{Model} & \textbf{Training} & \textbf{Overall} & \textbf{General} & \textbf{Adapt.} & \textbf{Challenge} & \textbf{MIEB} & \textbf{MMEB image} & \textbf{MMEB visdoc} \\
\midrule
Teacher CLIP & -- & XX.X & XX.X & XX.X & XX.X \\
CLIP-KD & Original & XX.X & XX.X & XX.X & XX.X \\

CLIP-KD & General & XX.X & XX.X & XX.X & XX.X \\

CLIP-KD & Gen.+Adapt. & XX.X & XX.X & XX.X & XX.X \\

TinyCLIP & Original & XX.X & XX.X & XX.X & XX.X \\

TinyCLIP & General & XX.X & XX.X & XX.X & XX.X \\

TinyCLIP & Gen.+Adapt. & XX.X & XX.X & XX.X & XX.X \\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table*}

\subsection{How Well Can Small Models Adapt?}

Table~\ref{tab:adaptability_results} focuses on the Adaptability group.
%
These tasks are below the TRACE threshold after General training, but have related training data available from MMEB or MIEB.
%
After adding the Adaptability training data, \textbf{CLIP-KD} improves from \textbf{XX.X} to \textbf{XX.X}, while \textbf{TinyCLIP} improves from \textbf{XX.X} to \textbf{XX.X}.
%
This shows that small CLIP models can benefit from in-domain data.
%
However, the gain varies across task types, indicating that adaptation is not uniform across the benchmark.

\begin{table}[h!]
\centering
\caption{
Adaptability results.
$\Delta$ denotes the improvement from adding related training data.
}
\label{tab:adaptability_results}
\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{l l c c c}
\toprule
\textbf{Model} & \textbf{Task Type} & \textbf{General} & \textbf{Gen.+Adapt.} & \textbf{$\Delta$} \\
\midrule
CLIP-KD & Retrieval & XX.X & XX.X & +XX.X \\
CLIP-KD & Classification & XX.X & XX.X & +XX.X \\
CLIP-KD & VQA / Choice & XX.X & XX.X & +XX.X \\
CLIP-KD & Grounding & XX.X & XX.X & +XX.X \\
CLIP-KD & Average & XX.X & XX.X & +XX.X \\
\midrule
TinyCLIP & Retrieval & XX.X & XX.X & +XX.X \\
TinyCLIP & Classification & XX.X & XX.X & +XX.X \\
TinyCLIP & VQA / Choice & XX.X & XX.X & +XX.X \\
TinyCLIP & Grounding & XX.X & XX.X & +XX.X \\
TinyCLIP & Average & XX.X & XX.X & +XX.X \\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table}

\subsection{Why Is the Challenge Group Difficult?}

Table~\ref{tab:challenge_analysis} breaks down the Challenge group by task type.
%
These tasks remain below the TRACE threshold after General training and do not have related training data available in the benchmark collection.
%
We observe that the lowest scores mainly come from \textbf{XXXXXX}.
%
This suggests that the Challenge group is not only difficult because of dataset format or metric choice.
%
Instead, it captures capabilities that are not sufficiently learned by current small CLIP training recipes, such as \textbf{XXXXXX}.

\begin{table}[h!]
\centering
\caption{
Breakdown of the Challenge group.
Small Avg. denotes the average score of small CLIP models, and Gap denotes the difference from the teacher.
}
\label{tab:challenge_analysis}
\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{l c c c c}
\toprule
\textbf{Task Type} & \textbf{\#Tasks} & \textbf{Small Avg.} & \textbf{Teacher} & \textbf{Gap} \\
\midrule
Retrieval & XX & XX.X & XX.X & XX.X \\
Classification & XX & XX.X & XX.X & XX.X \\
VQA / Choice & XX & XX.X & XX.X & XX.X \\
Grounding & XX & XX.X & XX.X & XX.X \\
Other & XX & XX.X & XX.X & XX.X \\
\midrule
Average & XX & XX.X & XX.X & XX.X \\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table}

\subsection{Gap between Large and Small Models}

Table~\ref{tab:teacher_student_gap} compares the large teacher with the small CLIP models.
%
Although distillation improves compact models, a clear gap remains.
%
The gap is smaller on the General group, where broad image-text data provides sufficient supervision.
%
In contrast, the gap is larger on the Adaptability and Challenge groups, showing that current small CLIP models still struggle to transfer the broader capability of the teacher.
%
These results suggest that improving small CLIP robustness requires more than optimizing retrieval performance.

\begin{table}[h!]
\centering
\caption{
Gap between the large teacher and small CLIP models.
We report the absolute score difference from the teacher.
}
\label{tab:teacher_student_gap}
\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{l l c c c c}
\toprule
\textbf{Model} & \textbf{Training} & \textbf{Overall} & \textbf{General} & \textbf{Adapt.} & \textbf{Challenge} \\
\midrule
CLIP-KD & Original & XX.X & XX.X & XX.X & XX.X \\
CLIP-KD & General & XX.X & XX.X & XX.X & XX.X \\
CLIP-KD & Gen.+Adapt. & XX.X & XX.X & XX.X & XX.X \\
TinyCLIP & Original & XX.X & XX.X & XX.X & XX.X \\
TinyCLIP & General & XX.X & XX.X & XX.X & XX.X \\
TinyCLIP & Gen.+Adapt. & XX.X & XX.X & XX.X & XX.X \\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table}


==> accv/5.tex <==
\section{Analysis}
\label{sec:analysis}

We further conduct diagnostic studies to understand why some tasks remain difficult under TRACE.
%
Rather than proposing a new training method, we analyze three factors that may affect small CLIP robustness: task prefix instructions, training hyperparameters, and teacher strength.
%
These studies help identify whether the Challenge group can be mitigated by simple training changes or whether it reflects a deeper limitation of current small CLIP recipes.

\subsection{Effect of Task Prefix Instructions}

Different TRACE tasks use different text formats, including captions, class labels, questions, answer choices, and task instructions.
%
This format mismatch may hurt small CLIP models, especially when the same text encoder is used across all tasks.
%
To study this effect, we compare models trained and evaluated with task-specific prefixes against models without prefixes.
%
Table~\ref{tab:prefix_ablation} shows that adding prefixes improves \textbf{XXXXXX}, suggesting that task instructions help align heterogeneous text inputs.
%
However, the improvement on the Challenge group remains limited, indicating that prefix formatting alone cannot fully explain the difficulty of these tasks.

\begin{table}[h!]
\centering
\caption{
Effect of task prefix instructions.
We compare models trained and evaluated with and without task-specific prefixes.
$\Delta$ denotes the improvement from using prefixes.
}
\label{tab:prefix_ablation}
\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{l c c c c}
\toprule
\textbf{Model} & \textbf{Prefix} & \textbf{General} & \textbf{Adaptability} & \textbf{Challenge} \\
\midrule
CLIP-KD & Without & XX.X & XX.X & XX.X \\
CLIP-KD & With & XX.X & XX.X & XX.X \\
CLIP-KD & $\Delta$ & +XX.X & +XX.X & +XX.X \\
\midrule
TinyCLIP & Without & XX.X & XX.X & XX.X \\
TinyCLIP & With & XX.X & XX.X & XX.X \\
TinyCLIP & $\Delta$ & +XX.X & +XX.X & +XX.X \\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table}

\subsection{Effect of Training Hyperparameters}

We next analyze whether the low performance on the Challenge group is caused by insufficient optimization.
%
Small CLIP models are usually trained with fixed recipes inherited from prior work, but TRACE contains more diverse tasks than standard retrieval benchmarks.
%
We therefore study simple hyperparameter changes, including longer training and learning-rate adjustment.
%
As shown in Table~\ref{tab:hyperparameter_ablation}, increasing the training budget or tuning the learning rate improves \textbf{XXXXXX}.
%
However, the gains are not uniform across groups.
%
This suggests that better optimization can improve adaptation, but it does not remove the robustness gap on Challenge tasks.

\begin{table}[h!]
\centering
\caption{
Effect of training hyperparameters.
We compare the default recipe with longer training and learning-rate adjustment.
}
\label{tab:hyperparameter_ablation}
\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{l l c c c c}
\toprule
\textbf{Model} & \textbf{Setting} & \textbf{Overall} & \textbf{General} & \textbf{Adaptability} & \textbf{Challenge} \\
\midrule
CLIP-KD & Default & XX.X & XX.X & XX.X & XX.X \\
CLIP-KD & More epochs & XX.X & XX.X & XX.X & XX.X \\
CLIP-KD & Tuned LR & XX.X & XX.X & XX.X & XX.X \\
\midrule
TinyCLIP & Default & XX.X & XX.X & XX.X & XX.X \\
TinyCLIP & More epochs & XX.X & XX.X & XX.X & XX.X \\
TinyCLIP & Tuned LR & XX.X & XX.X & XX.X & XX.X \\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table}

\subsection{Effect of Teacher Strength}

Finally, we examine whether a stronger teacher improves small CLIP robustness.
%
Knowledge distillation transfers the representation space of a large model to a compact student, so teacher quality may directly affect student performance.
%
We compare the default teacher with a stronger teacher while keeping the student architecture and training data fixed.
%
Table~\ref{tab:teacher_ablation} shows that a stronger teacher improves \textbf{XXXXXX}.
%
The largest gains appear on \textbf{XXXXXX}, while the Challenge group still shows a substantial remaining gap.
%
This indicates that teacher strength is important, but current distillation recipes may not fully transfer the broader capability of large CLIP models to small students.

\begin{table}[h!]
\centering
\caption{
Effect of teacher strength.
We compare small CLIP models distilled from the default teacher and a stronger teacher.
}
\label{tab:teacher_ablation}
\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{l l c c c c}
\toprule
\textbf{Model} & \textbf{Teacher} & \textbf{Overall} & \textbf{General} & \textbf{Adaptability} & \textbf{Challenge} \\
\midrule
CLIP-KD & Default & XX.X & XX.X & XX.X & XX.X \\
CLIP-KD & Stronger & XX.X & XX.X & XX.X & XX.X \\
CLIP-KD & $\Delta$ & +XX.X & +XX.X & +XX.X & +XX.X \\
\midrule
TinyCLIP & Default & XX.X & XX.X & XX.X & XX.X \\
TinyCLIP & Stronger & XX.X & XX.X & XX.X & XX.X \\
TinyCLIP & $\Delta$ & +XX.X & +XX.X & +XX.X & +XX.X \\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table}

Overall, these analyses show that task prefixes, optimization, and teacher strength can improve small CLIP models to some extent.
%
However, none of them fully resolves the Challenge group.
%
This supports the main motivation of TRACE: robust evaluation should distinguish tasks that are solved by general training, tasks that improve through adaptation, and tasks that remain open challenges for future small CLIP research.


==> accv/6.tex <==
\section{Conclusion}
\label{sec:conclusion}


In this paper, we introduced \textbf{TRACE}, a training-aware evaluation framework for small CLIP models.
%
Instead of evaluating compact vision-language models only by aggregate benchmark scores, TRACE organizes evaluation tasks according to their relationship with the training data.
%
This allows us to distinguish three cases: tasks that can be solved by broad image-text training, tasks that improve with related in-domain data, and tasks that remain challenging without available in-domain supervision.
%
By applying TRACE to MMEB and MIEB, we provide a more diagnostic evaluation protocol for understanding the robustness of small CLIP models beyond standard retrieval benchmarks.

Our study with CLIP-KD and TinyCLIP shows that current small CLIP models can achieve strong performance on the General group and benefit from related training data on the Adaptability group.
%
However, the Challenge group remains difficult even after controlled retraining.
%
This suggests that part of the improvement observed on broad embedding benchmarks comes from dataset-level adaptation, while some tasks still require capabilities that are not fully captured by current small CLIP training recipes.
%
Our analysis further shows that task prefixes, hyperparameter tuning, and stronger teachers can improve performance to some extent, but they do not fully close the gap on challenging out-of-domain tasks.

We hope TRACE encourages future work to evaluate small vision-language models in a more transparent and training-aware manner.
%
Future research can build on TRACE by developing better data selection strategies, stronger distillation objectives, and architectures that transfer the broader capability of large CLIP models more effectively.
%
Another important direction is to expand the Challenge group with new datasets and tasks, so that compact models can be evaluated not only for efficiency, but also for reliable generalization in real-world vision-language applications.


==> tables/adaptability_results.tex <==
\begin{table}[h!]
\centering
\caption{
Adaptability results.
$\Delta$ denotes the improvement from adding related training data.
}
\label{tab:adaptability_results}
\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{l l c c c}
\toprule
\textbf{Model} & \textbf{Task Type} & \textbf{General} & \textbf{Gen.+Adapt.} & \textbf{$\Delta$} \\
\midrule
\multirow{5}{*}{CLIP-KD} & Retrieval & 32.7 & 35.1 & +2.5 \\
 & Classification & 42.5 & 56.3 & +13.8 \\
 & VQA / Choice & 3.2 & 3.4 & +0.2 \\
 & Grounding & 34.5 & 39.2 & +4.7 \\
 & \bf{Average} & 34.8 & 42.5 & +7.7 \\
\midrule
\multirow{5}{*}{TinyCLIP} & Retrieval & 27.1 & 29.0 & +1.9 \\
 & Classification & 36.8 & 50.1 & +13.4 \\
 & VQA / Choice & 1.7 & 1.7 & +0.0 \\
 & Grounding & 39.3 & 41.5 & +2.2 \\
 & \bf{Average} & 30.1 & 37.2 & +7.1 \\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table}


==> tables/challenge.tex <==
\begin{table}[h!]
\centering
\caption{
Breakdown of the Challenge group.
Small Avg. denotes the average score of small CLIP models, and Gap denotes the difference from the teacher.
}
\label{tab:challenge_analysis}
\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{l l c c c c}
\toprule
\textbf{Model} & \textbf{Task Type} & \textbf{\#Tasks} & \textbf{Small Avg.} & \textbf{Teacher} & \textbf{Gap} \\
\midrule
\multirow{6}{*}{CLIP-KD} & Retrieval & 43 & 2.4 & 13.3 & 10.9 \\
 & Classification & 1 & 1.7 & 14.4 & 12.7 \\
 & VQA / Choice & 4 & 3.5 & 8.4 & 4.9 \\
 & Grounding & 0 & - & - & - \\
 & Other & 0 & - & - & - \\
 & \bf{Average} & 48 & 2.5 & 12.9 & 10.4 \\
\midrule
\multirow{6}{*}{TinyCLIP} & Retrieval & 43 & 1.7 & 15.9 & 14.2 \\
 & Classification & 1 & 1.2 & 14.4 & 13.2 \\
 & VQA / Choice & 4 & 3.0 & 8.8 & 5.8 \\
 & Grounding & 0 & - & - & - \\
 & Other & 0 & - & - & - \\
 & \bf{Average} & 48 & 1.8 & 15.3 & 13.5 \\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table}


==> tables/detailed_trace.tex <==
\begin{table*}[h!]
\centering

\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{l l c c c c c}
\toprule
\textbf{Category} & \textbf{Task Type} & \textbf{\#Tasks} & \textbf{CLIP-KD} & \textbf{TinyCLIP} & \textbf{MobileCLIP2-S0} & \textbf{CLIP ViT-B/16} \\
\midrule
\multirow{6}{*}{General} & Retrieval & 22 & 36.2 & 35.0 & 48.1 & 53.5 \\
 & Classification & 3 & 32.9 & 25.5 & 57.6 & 57.4 \\
 & VQA / Choice & 14 & 46.0 & 40.5 & 44.4 & 44.0 \\
 & Grounding & 0 & - & - & - & - \\
 & STS & 8 & 18.9 & 18.8 & 44.9 & 67.5 \\
 & \bf{Average} & 47 & 36.0 & 33.3 & 47.0 & 53.3 \\
\midrule
\multirow{6}{*}{Adapt.} & Retrieval & 28 & 33.4 & 29.9 & 40.6 & 48.0 \\
 & Classification & 33 & 42.6 & 40.5 & 62.0 & 62.7 \\
 & VQA / Choice & 6 & 3.1 & 2.5 & 3.1 & 4.9 \\
 & Grounding & 4 & 34.8 & 41.2 & 23.9 & 53.3 \\
 & STS & 0 & - & - & - & - \\
 & \bf{Average} & 71 & 35.2 & 33.1 & 46.4 & 51.5 \\
\midrule
\multirow{6}{*}{Challenge} & Retrieval & 44 & 2.2 & 1.5 & 6.9 & 18.5 \\
 & Classification & 2 & 2.3 & 5.7 & 13.5 & 20.6 \\
 & VQA / Choice & 3 & 2.2 & 2.7 & 3.0 & 9.0 \\
 & Grounding & 0 & - & - & - & - \\
 & STS & 1 & 2.2 & 0.4 & 37.7 & 60.3 \\
 & \bf{Average} & 50 & 2.2 & 1.7 & 7.5 & 18.9 \\
\bottomrule
\end{tabular}
\caption{Breakdown of Table~\ref{tab:main_results} by task type, showing the performance of the original models;
CLIP-KD and TinyCLIP define $\tau$ (pool A). Scores are means over the tasks on a 0-100 scale.}
\label{tab:detail_trace}
\vspace{-5mm}
\end{table*}

==> tables/teacher_student_gap.tex <==
\begin{table}[h!]
\centering
\caption{
Gap between the large teacher and small CLIP models.
We report the absolute score difference from the teacher. $^\dagger$Original TinyCLIP has no score for MSCOCO, RefCOCO, RefCOCO-Matching, Visual7W-Pointing; teacher compared on the same tasks.
}
\label{tab:teacher_student_gap}
\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{l l c c c c}
\toprule
\textbf{Model} & \textbf{Training} & \textbf{Overall} & \textbf{General} & \textbf{Adapt.} & \textbf{Challenge} \\
\midrule
\multirow{3}{*}{CLIP-KD} & Original & 15.1 & 20.1 & 14.7 & 10.7 \\
 & General & 15.2 & 20.5 & 14.6 & 10.4 \\
 & Gen.+Adapt. & 11.8 & 20.4 & 7.0 & 10.2 \\
\midrule
\multirow{3}{*}{TinyCLIP} & Original & 18.6$^\dagger$ & 23.0 & 19.2$^\dagger$ & 13.3 \\
 & General & 20.0 & 24.6 & 21.4 & 13.5 \\
 & Gen.+Adapt. & 16.6 & 23.4 & 14.3 & 13.2 \\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table}

